TFDNet: Time-Frequency Enhanced Decomposed Network for Long-term Time Series Forecasting

Long-term time series forecasting is a vital task and has a wide range of real applications. Recent methods focus on capturing the underlying patterns from one single domain (e.g. the time domain or the frequency domain), and have not taken a holistic view to process long-term time series from the time-frequency domains. In this paper, we propose a Time-Frequency Enhanced Decomposed Network (TFDNet) to capture both the long-term underlying patterns and temporal periodicity from the time-frequency domain. In TFDNet, we devise a multi-scale time-frequency enhanced encoder backbone and develop two separate trend and seasonal time-frequency blocks to capture the distinct patterns within the decomposed trend and seasonal components in multi-resolutions. Diverse kernel learning strategies of the kernel operations in time-frequency blocks have been explored, by investigating and incorporating the potential different channel-wise correlation patterns of multivariate time series. Experimental evaluation of eight datasets from five benchmark domains demonstrated that TFDNet is superior to state-of-the-art approaches in both effectiveness and efficiency.

==> Table/MACC.tex <==
% \begin{table*}[h]
% \centering
% \caption{The mean of absolute correlation coefficients among channels of original time series, seasonal components and trend components of 8 popular multivariate datasets. A higher value indicates stronger correlations between the channels.}
% \vspace{-1mm}
% \scalebox{0.80}{
% \begin{tabular}{cc|cccccccccccccccc}
% \toprule
% & Dataset &\multicolumn{1}{c|}{ETTm1}&\multicolumn{1}{c|}{ETTm2}&\multicolumn{1}{c|}{ETTh1}&\multicolumn{1}{c|}{ETTh2}&\multicolumn{1}{c|}{Electricity}&\multicolumn{1}{c|}{Traffic}&\multicolumn{1}{c|}{Weather}&\multicolumn{1}{c}{ILI}\\
% \midrule
% & Original & 0.335 & 0.420 & 0.333& 0.421 & 0.490 & 0.564 & 0.329 & 0.749 \\

% & Seaonsal & 0.302 & 0.369 & 0.352& 0.430 & 0.578 & 0.591 & 0.226 & 0.631 \\

% & Trend & 0.345 & 0.421 & 0.374 & 0.421 & 0.384 & 0.432 & 0.349 & 0.785 \\
% \bottomrule
% \end{tabular}
% \label{tab:MACC}
% }
% \end{table*}

\begin{table*}[!tb]
\centering
\caption{The mean of absolute correlation coefficients among different channels for the original multivariate time series and the decomposed trend and seasonal components on 8 datasets. A higher value (with deeper color) indicates stronger correlations between channels. }
%Seasonal and trend component each provide stronger relationships over the original on 8 popular multivariate datasets.}
\vspace{-1mm}
\scalebox{0.90}{
\begin{tabular}{cccccccccccccccccc}
\toprule
\textbf{Dataset} & \textbf{ETTm1}                & \textbf{ETTm2}                & \textbf{ETTh1}                & \textbf{ETTh2}                & \textbf{Electricity}          & \textbf{Traffic}              & \textbf{Weather}              & \textbf{ILI}                  \\ \midrule
Original  & \cellcolor[HTML]{B6E0C2}0.335 & \cellcolor[HTML]{B6E0C2}0.420  & \cellcolor[HTML]{FCFCFF}0.333 & \cellcolor[HTML]{B6E0C2}0.421 & \cellcolor[HTML]{A9DBB7}0.490  & \cellcolor[HTML]{B6E0C2}0.564 & \cellcolor[HTML]{B6E0C2}0.329 & \cellcolor[HTML]{B6E0C2}0.749 \\
Seaonsal  & \cellcolor[HTML]{FCFCFF}0.302 & \cellcolor[HTML]{FCFCFF}0.369 & \cellcolor[HTML]{B6E0C2}0.352 & \cellcolor[HTML]{63BE7B}0.430  & \cellcolor[HTML]{63BE7B}0.578 & \cellcolor[HTML]{63BE7B}0.591 & \cellcolor[HTML]{FCFCFF}0.226 & \cellcolor[HTML]{FCFCFF}0.631 \\
Trend     & \cellcolor[HTML]{63BE7B}0.345 & \cellcolor[HTML]{63BE7B}0.421 & \cellcolor[HTML]{63BE7B}0.374 & \cellcolor[HTML]{B6E0C2}0.421 & \cellcolor[HTML]{FCFCFF}0.384 & \cellcolor[HTML]{FCFCFF}0.432 & \cellcolor[HTML]{63BE7B}0.349 & \cellcolor[HTML]{63BE7B}0.785 \\ \bottomrule
\end{tabular}
\label{tab:MACC}
}
\end{table*}

% The mean of absolute correlation coefficients among channels of original time series, seasonal components and trend components of 8 popular multivariate datasets. A higher value (with deeper color) indicates stronger correlations between the channels.

==> Table/ab_moe.tex <==
\begin{table*}[tb]
\label{ablation_moe}
\caption{Ablation of MSTFT-MOE}
\centering
\vspace{-1mm}
\scalebox{0.7}{
\begin{tabular}{cc|llll|llll|llll}
\midrule
\multicolumn{2}{c|}{Datasets}                                  & \multicolumn{4}{c|}{Traffic}                                                                          & \multicolumn{4}{c|}{Electricity}                                                                               & \multicolumn{4}{c}{Weather}                                                                            \\ \midrule
\multicolumn{2}{c|}{Prediction Length T}                       & \multicolumn{1}{c}{96} & \multicolumn{1}{c}{192} & \multicolumn{1}{c}{336} & \multicolumn{1}{c|}{720} & \multicolumn{1}{c}{96}    & \multicolumn{1}{c}{192}   & \multicolumn{1}{c}{336}   & \multicolumn{1}{c|}{720}   & \multicolumn{1}{c}{96} & \multicolumn{1}{c}{192}   & \multicolumn{1}{c}{336} & \multicolumn{1}{c}{720} \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TFDNet-IK}}          & MSE & 0.377                  & 0.392                   & 0.406                   & 0.447                    & \textbf{0.128}            & \textbf{0.145}            & \textbf{0.160}            & \textbf{0.197}             & \textbf{0.143}         & \textbf{0.186}            & \textbf{0.236}          & 0.314                   \\
\multicolumn{1}{c|}{}                                    & MAE & 0.256                  & 0.263                   & 0.266                   & 0.287                    & \textbf{0.221}            & \textbf{0.237}            & \textbf{0.253}            & \textbf{0.285}             & \textbf{0.188}         & \textbf{0.230}            & \textbf{0.269}          & 0.326                   \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TFDNet-IK (Single)}} & MSE & 0.377                  & 0.393                   & 0.408                   & 0.449                    & 0.128 & 0.146                     & 0.162                     & 0.200                      & 0.144                  & 0.187                     & 0.237                   & \textbf{0.313}          \\
\multicolumn{1}{c|}{}                                    & MAE & 0.256                  & 0.264                   & 0.270                   & 0.290                    & 0.221 & 0.237                     & 0.254                     & 0.287                      & 0.189                  & 0.230         & 0.270                   & \textbf{0.325}          \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TFDNet-MK}}          & MSE & \textbf{0.354}         & \textbf{0.372}          & \textbf{0.388}          & \textbf{0.428}           & 0.129                     & 0.147                     & 0.163                     & 0.200                      & 0.148                  & 0.192                     & 0.243                   & 0.319                   \\
\multicolumn{1}{c|}{}                                    & MAE & \textbf{0.241}         & \textbf{0.250}          & \textbf{0.257}          & \textbf{0.279}           & 0.221           & 0.239                     & 0.256                     & 0.288                      & 0.194                  & 0.236                     & 0.275                   & 0.331                   \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TFDNet-MK (Single)}} & MSE & 0.361                  & 0.379                   & 0.394                   & 0.433                    & 0.130                     & 0.147                     & \multicolumn{1}{c}{0.164} & \multicolumn{1}{c|}{0.202} & 0.148                  & 193                   & 0.243                   & 0.317                   \\
\multicolumn{1}{c|}{}                                    & MAE & 0.246                  & 0.254                   & 0.261                   & 0.281                    & \multicolumn{1}{c}{0.222} & \multicolumn{1}{c}{0.239} & \multicolumn{1}{c}{0.256} & \multicolumn{1}{c|}{0.289} & 0.194                  & \multicolumn{1}{c}{0.236} & 0.276                   & 0.33                    \\ \bottomrule
\end{tabular}


}
\end{table*}

==> Table/ab_tf_structure.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h]
\centering
\caption{Ablation of time-frequency enhanced structure. Comparison of modeling in the time-frequency domain and single time domain (TimeNet) or frequency domain (FreqNet).  \textbf{Bold} indicates the best.}
\label{Ablation_tf}
\vspace{-1mm}
\scalebox{0.6}{
\begin{tabular}{@{}cc|llll|llll|llll|llll@{}}
\toprule
\multicolumn{1}{l}{Datasets}                    & \multicolumn{1}{l|}{} & \multicolumn{4}{c|}{Traffic}                                                                          & \multicolumn{4}{c|}{Electricity}                                                                      & \multicolumn{4}{c|}{Weather}                                                                          & \multicolumn{4}{c}{ETTm2}                                                                            \\ \midrule
\multicolumn{2}{l|}{Prediction Length T}                                & \multicolumn{1}{c}{96} & \multicolumn{1}{c}{192} & \multicolumn{1}{c}{336} & \multicolumn{1}{c|}{720} & \multicolumn{1}{c}{96} & \multicolumn{1}{c}{192} & \multicolumn{1}{c}{336} & \multicolumn{1}{c|}{720} & \multicolumn{1}{c}{96} & \multicolumn{1}{c}{192} & \multicolumn{1}{c}{336} & \multicolumn{1}{c|}{720} & \multicolumn{1}{c}{96} & \multicolumn{1}{c}{192} & \multicolumn{1}{c}{336} & \multicolumn{1}{c}{720} \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TFDNet-IK}} & MSE                   & 0.377                  & 0.392                   & 0.406                   & 0.447                    & \textbf{0.128}         & \textbf{0.145}          & \textbf{0.160}          & \textbf{0.197}           & \textbf{0.143}         & \textbf{0.186}          & \textbf{0.236}          & \textbf{0.314}           & \textbf{0.157}         & \textbf{0.213}          & \textbf{0.264}          & \textbf{0.345}          \\
\multicolumn{1}{c|}{}                           & MAE                   & 0.256                  & 0.263                   & 0.266                   & 0.287                    & \textbf{0.221}         & \textbf{0.237}          & \textbf{0.253}          & \textbf{0.285}           & \textbf{0.188}         & \textbf{0.230}          & \textbf{0.269}          & \textbf{0.326}           & \textbf{0.244}         & \textbf{0.282}          & \textbf{0.318}          & \textbf{0.371}          \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TFDNet-MK}} & MSE                   & \textbf{0.354}         & \textbf{0.372}          & \textbf{0.388}          & \textbf{0.428}           & 0.129                  & 0.147                   & 0.163                   & 0.200                    & 0.148                  & 0.192                   & 0.243                   & 0.319                    & 0.158                  & 0.214                   & \textbf{0.264}          & 0.347                   \\
\multicolumn{1}{c|}{}                           & MAE                   & \textbf{0.241}         & \textbf{0.250}          & \textbf{0.257}          & \textbf{0.279}           & \textbf{0.221}         & 0.239                   & 0.256                   & 0.288                    & 0.194                  & 0.236                   & 0.275                   & 0.331                    & 0.246                  & 0.283                   & 0.319                   & 0.372                   \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{FreqNet}}  & MSE                   & 0.385                  & 0.396                   & 0.409                   & 0.446                & 0.136                  & 0.149                   & 0.165                   & 0.204                    & 0.165                  & 0.207                   & 0.256                   & 0.322                    & 0.158                  & 0.214                   & 0.265                   & 0.351                   \\
\multicolumn{1}{c|}{}                           & MAE                   & 0.260                  & 0.264                   & 0.270                   &0.290                          & 0.229         & 0.240                   & 0.257                   & 0.290                    & 0.212                  & 0.249                   & 0.286                   & 0.334                    & 0.246                  & 0.287                   & 0.320                   & 0.376                   \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{TimeNet}} & MSE                   & 0.393                  & 0.403                   & 0.415                   & 0.453                    & 0.136                  & 0.148                   & 0.164                   & 0.203                    & 0.169                  & 0.212                   & 0.258                   & 0.326                    & 0.159                  & 0.215                   & 0.268                   & 0.353                   \\
\multicolumn{1}{c|}{}                           & MAE                   & 0.262                  & 0.265                   & 0.271                   & 0.291                    & 0.230                  & 0.240                   & 0.257                   & 0.289                    & 0.215                  & 0.252                   & 0.288                   & 0.338                    & 0.247                  & 0.286                   & 0.322                   & 0.376                   \\ \bottomrule
\end{tabular}
}
\end{table*}

==> Table/noise.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Noise injection experiments. A $0.3 \mathcal{N}(0,1)$ Gaussian noise is injected into the training and testing dataset. We conduct 4 sets with/without noise on ETTh1 datasets with different output lengths. The relative value of the metric is shown ('+'/'-' indicates worse/better performance).}
\scalebox{0.8}{
\vspace{-1mm}
% \scalebox{0.60}{
\begin{tabular}{@{}cc|cccccccc@{}}
\toprule
\multicolumn{2}{c|}{Training}                         & \multicolumn{4}{c|}{with noise}                                      & \multicolumn{4}{c}{without noise}                                   \\ \midrule
\multicolumn{2}{c|}{Testing}                          & \multicolumn{2}{c|}{with noise} & \multicolumn{2}{c|}{without noise} & \multicolumn{2}{c|}{with noise} & \multicolumn{2}{c}{without noise} \\ \midrule
\multicolumn{2}{c|}{Metric}                           & MSE            & MAE            & MSE              & MAE             & MSE            & MAE            & MSE             & MAE             \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{TDFNet-IK}} & 96  & +1.20\%        & +1.19\%        & -2.20\%          & -1.83\%         & +2.00\%        & +1.90\%        & 0.359           & 0.386           \\
\multicolumn{1}{c|}{}                           & 192 & +1.00\%        & +0.83\%        & -1.83\%          & -1.25\%         & +1.17\%        & +0.82\%        & 0.398           & 0.412           \\
\multicolumn{1}{c|}{}                           & 336 & +0.48\%        & +0.45\%        & -1.34\%          & -0.66\%         & +0.33\%        & +0.08\%        & 0.432           & 0.431           \\
\multicolumn{1}{c|}{}                           & 720 & +0.74\%        & +0.41\%        & -2.04\%          & -0.87\%         & +1.25\%        & +0.99\%        & 0.438           & 0.453           \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{TDFNet-MK}} & 96  & +1.36\%        & +1.48\%        & -2.26\%          & -2.13\%         & +2.43\%        & +2.67\%        & 0.356           & 0.383           \\
\multicolumn{1}{c|}{}                           & 192 & +1.09\%        & +1.07\%        & -2.20\%          & -1.77\%         & +1.40\%        & +1.58\%        & 0.396           & 0.409           \\
\multicolumn{1}{c|}{}                           & 336 & +0.64\%        & +0.62\%        & -1.55\%          & -0.92\%         & +1.18\%        & +0.78\%        & 0.431           & 0.429           \\
\multicolumn{1}{c|}{}                           & 720 & +1.22\%        & +1.00\%        & -1.72\%          & -1.07\%         & +1.31\%        & +0.97\%        & 0.421           & 0.443           \\ \bottomrule
\end{tabular}
\label{tab:noise}
}
\end{table*}

==> draft.tex <==
\section{Time Series Representation in Time-Frequency Domain}


\subsection{The Limitations of Single Domain}
Recently research illustrates that time series data can be modeled through the time domain and frequency domain. However, the conventional representations in the time domain or frequency domain are inadequate \citep{boashash2015time}. Any time series can be described as a function of time, but the model using time-domain representation is difficult to preserve the overall characteristics and statistical properties of time series.  Meanwhile, time domain analysis may not be able to capture the underlying frequency information in the data. This means that some important features of the data, such as periodicity, may be missed. Frequency-domain representation is wildly used in time series analysis  and it can better capture the global properties of the signal  than time-domain representation \citep{zhou2022fedformer}. As Fourier transform, a common tool to transform time series from the time domain to the frequency domain, there are also defects. The frequency spectrum obtained after the Fourier transform does not contain any information about the time at which events and frequencies occur or their duration \citep{boashash2015time}. 

\subsection{Short Time Fourier Transform}
Given the limitations of conventional representations in either the time domain or frequency domain, the representation of a two-variable function or distribution in a two-dimensional space is more applicable in time series analysis.
Such a representation is called a time-frequency representation (TFR) 
 \cite{boashash2015time}.  TFR can be obtained by time-frequency transforms including the short-time Fourier transform (STFT), the continuous wavelet transform (CWT), and the discrete wavelet transform (DWT). 
 
 
 Unlike previous studies  \citep{zhang2022tfad}, we use STFT as the main method to represent time-frequency features. The reasons that STFT is more suitable for time series forecasting are: (1) STFT can provide accurate phase information, which helps to analyze the timing characteristics of the series. In contrast, DWT only provides amplitude information and no phase information.  (2)
 

==> section/1_introduction-old.tex <==
\section{Introduction}
\ziyu{all symbols should be defined in the symbols.tex}
\ziyu{Rewrite Introduction part}
Time series analysis encompasses a variety of crucial undertakings, among which long-term time series forecasting (LTSF) stands out as particularly pivotal. LTSF holds significant implications across numerous domains, including but not limited to energy, weather, economics, and transportation \cite{rajagukguk2020review,angryk2020multivariate,sezer2020financial,chen2019review}. The immense practical utility of LTSF has spurred a surge of interest in this field. 
% With the swift advancement of deep learning technology, neural network designs have been in the context of \textbf{TSF} \cite{wen2022transformers} \cite{lim2021time}. 

% In contrast to conventional forecasting tasks, LTSF is beset by formidable hurdles such as protracted temporal dependencies, vulnerability to error amplification, intricate patterns, and nonlinear dynamics \cite{zhou2022film}. With the swift advancement of deep learning technology, neural network designs have been used to address these challenges in the context of LTSF. The Transformer model \cite{vaswani2017attention} has demonstrated notable achievements in the fields of Natural Language Processing (NLP) \cite{vaswani2017attention,devlin2018bert}\ziyu{add citations} and Computer Vision (CV) \cite{dosovitskiy2020image,liu2021swin} \ziyu{add citations}. Furthermore, it exhibits encouraging outcomes in effectively capturing prolonged dependencies in the context of time series prediction \cite{wu2021autoformer,zhou2022fedformer,lim2021time}. Meanwhile, some non-transformer-based models with special structures also demonstrate excellent performance \cite{zhou2022film,zeng2022transformers,liu2022scinet,wu2022timesnet}.
It is well-known that time series data can be represented in the time domain and frequency domain \cite{broomhead1989time}. We notice that most of the LSTF models are modeled in a singular domain. For example, Autoformer \cite{wu2021autoformer} and PatchTST \cite{nie2022time} are modeled in the time domain, meanwhile FEDformer \cite{zhou2022fedformer} and FiLM \cite{zhou2022film} are modeled in the frequency domain. However, the representations in the time domain or frequency domain are inadequate \cite{boashash2015time}. Time domain analysis may not be able to capture the underlying frequency information in the data. This means that some important data features, such as periodicity, may be missed \cite{sun2022fredo}. Frequency-domain representation is wildly used in time series analysis  and it can better capture the global properties of the signal  than time-domain representation \citep{zhou2022fedformer}. The Fourier transform \cite{boashash2015time} is a common tool to transform time series from the time domain to the frequency domain. However, the frequency spectrum obtained after the Fourier transform does not contain any information about the time at which events and frequencies occur or their duration \citep{boashash2015time}. In order to make full use of the information in both time and frequency dimensions, we utilize Short-time Fourier transform (STFT) \cite{boashash2015time} to represent the time series in the time-frequency domain and develop kernels to obtain the historical information. 

The channel-independence (CI) strategy \cite{nie2022time,zeng2022transformers} means that each input series only contain the information from the single channel, and it is proven more robust and accurate results in time series predictions \cite{han2023capacity}. By comparison, the channel-mixing (CM) strategy embeds the whole channels into high-dimensional vectors. As for the CM strategy, the embedding vectors are considered to represent the entire information of all channels. In this case, CM models employ a group of parameters $\theta$ to be on behalf of the distribution $P_{\theta}(\mathcal{\outputseq}|\mathcal{\inputseq})$, where $\mathcal{\inputseq}$ is the input sequence of all channels and $\mathcal{\outputseq}$ is the predictions. Whereas, as for the CI models each channel shares the same parameters, which means $P_{\theta}(\mathcal{\outputseq}_a|\mathcal{\inputseq}_a)=P_{\theta}(\mathcal{\outputseq}_b|\mathcal{\inputseq}_b)$ where $a,b$ donates two different channels. However, is it really reasonable to consider that they have the same distributions among all channels? This question depends on the inherent characteristics of the time series dataset. Regarding correlation, in cases where there are high correlations among data channels, utilizing shared parameters can facilitate generalization across all channels. However, in cases where the channel correlations of the time series are low, it is more justifiable to utilize individual parameters. The utilization of seasonal-trend decomposition of time is a prevalent technique for analysis \cite{rojo2017modeling,wu2021autoformer}. Upon decomposing the time series, it has been observed that the correlation of the channel has exhibited variations.
\input{Table/MACC.tex}
Table \ref{tab:MACC} illustrates the mean of absolute channel correlation coefficient of 8 popular multivariate datasets provided in \cite{wu2021autoformer}. The seasonal components typically show more complex patterns and frustration \cite{wang2023micn}, so we focus on these parts. Some time series data demonstrate lower correlations in the seasonal component compared with the original data like Weather. For these datasets, it is possible to assert that the seasonal part exhibits a greater amount of distinctive information across channels. Meanwhile, other datasets like Traffic exhibit stronger correlations in seasons, thereby augmenting their mutual information.
% We use MACC to measure the correlation among channels of each dataset, and it shows that they have various correlations in the full series, trend parts, and seasonal parts. In this situation, it is reasonable to share the same parameters among channels of the dataset with a high correlation like Traffic. However, it is more proper to set individual parameters in the model of datasets with a low correlation like Weather. In the empirical analysis, each channel in the Traffic dataset means the road occupancy rates measured in different locations, and their variations always exhibit the same regularity with time. However, in the Weather dataset, each channel donates differing meteorological indicators such as air temperature, atmospheric pressure intensity, etc, and there is no obvious correlation between some indicators. 

Based on the above motivations, we propose a \textbf{T}ime-\textbf{F}requency \textbf{E}hanced \textbf{D}ecomposed
\textbf{N}etwork (\textbf{TFDNet}) for LSTF. TFDNet uses Multi-Scale STFT (MSTFT) to obtain the time-frequency matrixes of diverse resolutions. Our model decomposes the input sequence into the trend component and the seasonal component processing them through Trend Encoder and Seasonal Encoder with Time-frequency Block (TFB). Seasonal Encoder employs Seasonal TFB (STFB), which has two subversions: STFB Individual Kernel (STFB-IK) and STFB Multiple Kernel (STFB-MK). STFB-IK with individual parameters across channels and STFB-MK with shared parameters address two scenarios in which time series displays differential information and common information pertaining to seasonal items. Trend Encoder utilizes the Trend TFB (TTFB) to process the trend component. TFDNet achieves state-of-the-art accuracy on five benchmarks. The contributions are summarized as follows:   
% Considering the difference among channels and the seasonal component demonstrates a lower correlation We provide two versions, TFDNet-IK and TFDNet-MK. TFDNet-IK has a Time-frequency Block Individual Kernels (STFB-IK) with individual parameters in the seasonal encoder of each channel to process the seasonal trend with low correlation, and TFDNet-MK has a Time-frequency Block Multiply Kernels (STFB-MK) with multiple kernels sharing the same parameters to process the seasonal trend with high correlation. The trend encoder includes a Trend Time-Frequency Block (TTFB). Another reason that the trend component and seasonal component have different configurations is that we notice the seasonal component always shows more complex and diverse variations than the trend component \cite{wang2023micn,zhang2022first}. TFDNet achieves state-of-the-art accuracy on five benchmarks. The contributions are summarized as follows:
\begin{enumerate}
\setlength{\parskip}{0.05pt}
    \item We propose a {\it Time-Frequency Ehanced Decomposed
    Network} architecture with s seasonal-trend decomposition and Multi-Scale STFT for more accurate predictions of long-term time series.
    \item We propose {\it Trend Time-frequency Bock} in the trend encoder and {\it Seasonal Time-frequency Bock} in the seasonal encoder to capture the historical information through time-frequency mapping.
    \item We propose the channel correlation question for the CI strategy. In this case, we design individual parameter kernels for datasets with low channel correlations and shared multiple kernels for datasets with high channel correlations.
    % \item We conduct extensive experiments on six benchmark datasets across multiple domains (energy, traffic, economics, weather, and disease). Our empirical studies show that the proposed model improves the performance of state-of-the-art methods by \textbf{19.2\%} and \textbf{26.1\%} in multivariate and univariate forecasting, respectively. In addition, our empirical studies also reveal a dramatic improvement in computational efficiency through dimensionality reduction. 
    \item Our TFDNet has been demonstrated to be highly effective and efficient in comparison to previous state-of-the-art models with extensive experimentation on five real-world benchmarks.
\end{enumerate}

% The models can be categorized into two distinct classes: iterated multi-step (\textbf{IMS}) forecasting and direct multi-step (\textbf{DMS}) forecasting \cite{zeng2022transformers}.  It is well known that \textbf{IMS} forecasting is susceptible to substantial error accumulation effects when applied to the LTSF problem. Despite its limitations, \textbf{DMS} forecasting models have demonstrated considerable efficacy in capturing long-term dependencies in sequential data. The predominant form of direct multi-step \textbf{DMS} forecasting models are those based on Transformer \cite{vaswani2017attention} architectures, i.e., Informer \cite{zhou2021informer}, Autoformer \cite{wu2021autoformer}, Fedformer \cite{zhou2022fedformer}, and the recent PatchTS \cite{nie2022time}. There are also other models like FILM \cite{zhou2022film}6
% and DLinear \cite{zeng2022transformers} of non-transformer-based architectures that demonstrate good performance in \textbf{LTSF}. It is worth noting that non-transformer-based architectures such as FILM \cite{zhou2022film}, DLinear \cite{zeng2022transformers}, and TimesNet \cite{wu2022timesnet} have also exhibited strong performance in the context of \textbf{LTSF}.
















==> section/3_background.tex <==
% \section{Background}
% \subsection{Time Series Representation in Time-Frequency Domain}
Recently research has illustrated that time series data can be modeled through the time domain and frequency domain \cite{boashash2015time}. However, the conventional representations in the time domain or frequency domain are inadequate \cite{boashash2015time} \cite{zhang2022tfad}. In this case, the representation of a two-variable function or distribution in a two-dimensional space is more applicable in time series analysis. Such a representation is called a time-frequency representation. The Short-Time Fourier Transform (\textbf{STFT}) is a well-established method employed to analyze the frequency content of a non-stationary signal and observe its temporal evolution \cite{parchami2016recent}. \textbf{STFT} enables the transformation of time series from the time domain to the time-frequency domain. And the resulting representation of the \textbf{STFT} is a 2D matrix that is amenable to straightforward processing. When compared to\textbf{STFT}, the Discrete Wavelet Transform (\textbf{DWT}), a commonly used time-frequency transform in time series analysis, transforms the input sequence into vectors of varying dimensions via high and low pass filters, which can result in a representation that is more challenging to process than the 2D matrix produced by \textbf{STFT}.  In this paper, we use \textbf{STFT} to build the time-frequency representation $X[\omega,m]$ of input sequence $x$, as the following
\begin{equation}
    X[\omega,m]= \sum^{N-1}_{k=0} w[n] x[n+ml]e^{-j\frac{2\pi\omega}{N}}
\end{equation}
Here, $w[n]$ refers to the window utilized to extract a frame from the complete sequence, where $k$ denotes the index within each frame, $N$ denotes the window length, $l$ represents the frameshift, and $\omega$ and $m$ respectively denote the frequency bins and index of the sliding window. In essence,  \textbf{STFT} can be viewed as a technique that involves computing the Discrete Fourier Transform (\textbf{DFT}) of each frame in a signal, which is obtained by applying a sliding window to the original time series.

\subsection{Channel-independence and 2D Representation}
% Channel-independence means the characteristic where every input token solely comprises information from a singular channel \cite{nie2022time}. Recent research has demonstrated the efficacy of channel-independence in \textbf{LTSF} \cite{zeng2022transformers} \cite{nie2022time}.
% With channel-independence, the input is a 1D sequence of time series for each channel rather than a 2D matrix in channel-mixing. In this case, for a better representation of the 1D input, there is a method that transforms the 1D data into the 2D form \cite{wu2022timesnet}. The new dimension can illustrate a new perspective of temporal variation, for example, TimesNet \cite{wu2022timesnet} uses a 2D matrix to present the intraperiod-variation and interperiod-variation successfully. 

According to Nie et al. \cite{nie2022time}, channel-independence is characterized by input tokens that contain information from a singular channel exclusively. Recent studies, including those by Zeng et al. \cite{zeng2022transformers} and Nie et al. \cite{nie2022time}, have demonstrated the effectiveness of channel-independence in \textbf{LTSF}. Instead of using a 2D matrix with channel dimension and time dimension in channel-mixing, channel-independence employs a 1D sequence of time series for each channel. To achieve a better representation of the 1D input sequence, Wu et al. \cite{wu2022timesnet} proposed a method that transforms the 1D data into a 2D format. The additional dimension provides a new perspective on temporal variation, as exemplified by TimesNet \cite{wu2022timesnet}, which utilizes a 2D matrix to successfully represent both intraperiod-variation and interperiod-variation.

Notably, time series data inherently exhibits two dimensions: one in the time domain and the other in the frequency domain. To provide an efficient and multidimensional representation of time series, we propose a novel approach that utilizes STFT to transform non-stationary time series data. This method extends the original 1D sequence into a 2D time-frequency matrix, which effectively captures the time and frequency information of the input data. In our proposed method, the time-frequency matrix encompasses the frequency information of each time frame. Additionally, in the time domain, it effectively illustrates the variation of frequency across different durations.





    
Any time series can be described as a function of time, but the model using time-domain representation is difficult to preserve the overall characteristics and statistical properties of time series.  Meanwhile, time domain analysis may not be able to capture the underlying frequency information in the data. This means that some important data features, such as periodicity, may be missed. Frequency-domain representation is wildly used in time series analysis  and it can better capture the global properties of the signal  than time-domain representation \citep{zhou2022fedformer}. As Fourier transform, a common tool to transform time series from the time domain to the frequency domain, there are also defects. The frequency spectrum obtained after the Fourier transform does not contain any information about the time at which events and frequencies occur or their duration \citep{boashash2015time}. 
